Coalgebraic Automata Theory: Basic Results

We generalize some of the central results in automata theory to the abstraction level of coalgebras and thus lay out the foundations of a universal theory of automata operating on infinite objects. Let F be any set functor that preserves weak pullbacks. We show that the class of recognizable languages of F-coalgebras is closed under taking unions, intersections, and projections. We also prove that if a nondeterministic F-automaton accepts some coalgebra it accepts a finite one of the size of the automaton. Our main technical result concerns an explicit construction which transforms a given alternating F-automaton into an equivalent nondeterministic one, whose size is exponentially bound by the size of the original automaton.

==> prel.tex <==
\newcommand{\pwE}{\Pow_{\elo}}
\newcommand{\pwA}{\Pow_{\abe}}

\section{Preliminaries}
\label{s:2}

Since coalgebra automata bring together notions from two research areas
(coalgebra and automata theory), we have made an effort to make this paper
accessible to both communities.
As a consequence, we have included a fairly long section containing the
background material that is needed for understanding the main definitions and
proofs of the paper.
Readers who want to acquire more knowledge could consult
\textsc{Rutten}~\cite{rutt:univ00} and 
\textsc{Gr\"{a}del, Thomas \& Wilke}~\cite{grae:auto02}
for further details on universal coalgebra and automata theory, respectively.
For a more gentle introduction to coalgebra automata, the reader is referred
to \textsc{Venema}~\cite{vene:xxxx06}.

\subsection{Coalgebras, bisimulations and relation lifting}

Informally, a coalgebra consists of a set $S$ of \emph{states}, together
with a \emph{transition structure} $\si$ mapping a state $s \in S$ to an
object $\si(s)$ in the set $\F S$, where $\F$ is the \emph{type} of the 
structure $\bbS$.
Technically, the type of a coalgebra is formalized as a \emph{set functor},
i.e. an endofunctor on the category $\Set$ having sets as objects and 
functions as arrows.
Such a functor maps a set $S$ to a set $\F S$, and a function $f: S \to S'$
to a function $\F f: \F S \to \F S'$.

\begin{definition}
Given a set functor $\F$, an $\F$-coalgebra is a pair $\bbS =
\struc{S,\si}$ with $\si: S \to \F S$.
A \emph{pointed coalgebra} is a pair consisting of a coalgebra together
with an element of (the carrier set of) that coalgebra.
\end{definition}

\newcommand{\probdist}{\mathsf{D}}
\newcommand{\multiset}{\mathsf{M}}

\begin{example}
\label{ex:BTK}
\begin{enumerate}
\item For instance, consider the functor $\BT$ which associates with a set $S$
the cartesian product $S \times S$, and with a map $f: S \to S'$, the map
$\BT f: S\times S \to S'\times S'$ given by $(\BT f)(s,s') := 
(f(s),f(s'))$.
Thus every state in an $\BT$-coalgebra has both a left and a right
successor.
As a special example of a $\BT$-coalgebra, consider the \emph{binary tree}
given as the set $2^{*}$ of finite words over the alphabet $2 =
\{0,1\}$, with the coalgebra map given by $s \mapsto (s0,s1)$.

\item Directed graphs can be seen as coalgebras of the power set functor $\K$.
(The notation is mnemonic of the fact that in the present coalgebraic context, 
directed graphs are better known as \emph{Kripke frames}.)
The functor $\K$ maps a set to its collection of subsets, and a function
$f: S \to S'$ to its direct image function $\K f: \power S \to \power S'$
given by $(\K f)(X) := \{ f(x) \in S' \mid x \in X \}$.
A graph $(G,E)$ is then modelled as the coalgebra $(G,\lambda x.E[x])$,
that is, the relation $E$ is given by the function mapping a point $x$ to 
the collection $E[x]$ of its (direct) successors.

\item In general, given a functor $\F$, we denote with $\F_{C}$ the functor 
given by $\F(S) = C \times \F S$.
So $\BT_{C}$ and $\K_{C}$ are, respectively, the functors that we may 
associate with $C$-labelled binary trees and $C$-labelled graphs,
respectively. 
%\end{example}



%\begin{example}
\item Let
$\probdist$ be the functor that maps a set $S$ to the set
\[ \probdist S \coloneqq \left\{ \rho: S \to [0,1] \mid \rho
\; \mbox{has finite support and} \; \sum_{s\in S} 
\rho(s) = 1\right\} \]
where we say that $\rho$ has finite support if  $\rho(s) \not= 0$
for only finitely many elements $s$ of $S$. Then 
coalgebras for the functor $1 + \probdist$
correspond to probabilistic transition systems 
which have been introduced
by Larsen and Skou in~\cite{laskou:prob}. Here $1 + \probdist$ denotes
the functor that maps a set $S$ to the disjoint union of the one-element set
and the set $\probdist S$. Further details about this example can be
found in \cite{moss:coal99} and \cite{vinkrut:prob}.

\item Transition systems in which every state
has a {\em multiset} of successors are coalgebras for the functor
$\multiset$ that maps a set $S$ to the set $\multiset S$ of all
functions $\mu: S \to \bbN$ that have finite support, i.e.\
$\mu(s) \not= 0$ for only finitely many elements $s$ of $S$.
More information can be found in~\cite{gumm:moinoid}

\end{enumerate}
\end{example}
\begin{remark}
The action of $\F$ on functions is needed to define the \emph{morphisms}
between two coalgebras (which will not be needed in this paper).
Formally, given two $\F$-coalgebras $\bbS = \struc{S,\si}$ and $\bbS' = 
\struc{S',\si'}$, a function $f: S \to S'$ is a coalgebra morphism if 
$\si'\circ f = (\F f) \circ \si$.
\end{remark}

\begin{remark}
It will be very convenient for us to confine our attention to the so-called
\emph{standard} functors.
A functor is \emph{standard} if it turns inclusion maps into inclusions;
in particular, this means that $A' \sse A$ implies $\F A' \subseteq \F A$.
Not every functor is standard (for an example, one may consider the functor
taking a set $S$ to the collection of filters over $S$, and a map $f$ to
its double inverse image map $(f^{-1})^{-1}$).
%
%recall that a \emph{filter}}
%over a set $S$ is a collection $F \sse \Sb{S}$ which is closed under taking
%intersection and supersets.
%Now consider the functor that sends a set $S$ to the collection 
%$\mathit{Fil}(S)$ of all filters over $S$, and a map $f: S \to S'$ to the
%map $(f^{-1})^{-1}$ obtained by taking inverse image twice.
%Now suppose that 
%
%
Fortunately however, one may show that 
\shtbs{every standard functor is \ldots}
While the results of this paper apply to standard and non-standard functors
alike, for a smooth presentation we will always assume that the functors we 
are dealing with are standard.
\end{remark}

As mentioned in the introduction, the theory of coalgebra aims to provide
a simple but general framework for formalizing and studying the concept of
\emph{behavior}.
For this purpose it is of importance to develop a notion of \emph{behavioral
equivalence} between states.
For almost all important coalgebraic types, this notion can be naturally
expressed using \emph{bisimulations}.
Intuitively, these are relations between the state sets of two coalgebras 
that witness the observational indistinguishability of the pairs that they
relate.
For our purposes it will be convenient to use a definition of bisimilarity
in terms of \emph{relation lifting}.

\begin{definition}
\label{d:rellift}
Let $\F$ be a set functor.
Given two sets $S$ and $S'$, and a binary relation $Z$ between $S
\times S'$, we define the relation $\Fb (Z) \sse \F S \times \F
S'$
as follows:
\[
\Fb (Z) := \{ ((\F\pi) \phi, (\F\pi')\phi) \mid \phi \in \F Z \},
\]
where $\pi: Z \to S$ and $\pi':Z \to S'$ are the projection functions given
by $\pi(s,s') = s$ and $\pi'(s,s') = s'$.
\shtbs{Diagram to be added}

Now let $\bbS = \struc{S,\si}$ and $\bbS' = \struc{S',\si'}$ be two 
$\F$-coalgebras.
Then a relation $Z \sse S \times S'$ satisfying
\begin{equation}
\label{eq:bis}
(\si(s),\si'(s')) \in \Fb(Z)
\mbox{ for all } (s,s') \in Z.
\end{equation}
is a \emph{bisimulation} between $\bbS$ and $\bbS'$.
Two states are \emph{bisimilar} iff they are linked by some bisimulation.
\end{definition}

Intuitively, for $Z \sse S \times S'$ to be a bisimulation we require 
that whenever $s$ and $s'$ are linked by $Z$, then $\si(s)$ and $\si'(s)$
are linked by the lifted version $\Fb(Z)$ of $Z$.

\begin{example}
Let's see how these definitions apply to coalgebras for the functors 
$\BT_{C}$ and $\K$ of Example~\ref{ex:BTK}.
For this purpose, fix two sets $S$ and $S'$, and a relation $Z \sse S \times S'$.

For the definition of the relation $\ovl{\BT_{C}}(Z)$, it is easy to see that 
$(c,s_{0},s_{1})$ and $(c',s_{0}',s_{1}')$ are related iff $c = c'$ and
both $(s_{0},s_{0}')$ and $(s_{1},s_{1}')$ belong to $Z$.
Hence the relation $Z$ is a bisimulation between two $\BT_{C}$-coalgebras 
if $Z$-related points have the same color and both their left successors
and their right successors are $Z$-related.
From this it easily follows that two labelled binary trees are bisimilar iff
they are identical.
However, the notion becomes less trivial if we consider other coalgebras for
the functor $\BT_{C}$.
In fact, bisimilarity can be used to formulate some well-known notions in the
theory of tree automata; for instance, a labelled binary tree is 
\emph{regular} iff it is bisimilar to a finite $\BT_{C}$-coalgebra.

Concerning the Kripke functor $\K$, observe that $(X,X') \in \ovl{\K}(Z)$ iff
for all $x \in X$ there is an $x' \in X'$, and for all $x' \in X'$ there is
an $x \in X$ such that $(x,x') \in Z$.
That is, $\ovl{\K}(Z)$ is the \emph{Egli-Milner} lifting of $Z$.
Thus, a relation relating nodes of one graph $\bbS$ to those of another
graph $\bbS'$ is a \emph{bisimulation} if for every linked pair $(s,s')$,
every successor $t$ of $s$ is related to some successor $t'$ of $s'$, and,
vice versa, every successor $t'$ of $s'$ is related to some successor $t$ of
$s$.

Finally, the connection between $\Fb$ and $\ovl{\F_{C}}$ is given by the
following: $((c,\phi),(c',\phi')) \in \ovl{\F_{C}}(Z)$ iff $c=c'$ and 
$(\phi,\phi') \in \Fb(Z)$.
\end{example}


%\begin{remark}
%\label{r:bis}
%Formally, a relation $Z \sse S\times S'$ is a bisimulation between
%two coalgebras $\bbS$ and $\bbS'$ iff we may endow $Z$ with a 
%coalgebra structure $\zeta: Z \to \F Z$ such that the two projection
%functions $\pi_{i}: Z \to S_{i}$ are coalgebra morphisms.
%\end{remark}

Given the key role that relation lifting plays in this paper, we need some
of its properties.
It can be shown that relation lifting interacts well with the operation 
taking the graph $\Graph{f} := \{ (s,s') \in S \times S' \mid f(s) = s' \}$ 
of a function $f: S \to S'$, and with most operations on binary relations.
In fact, the properties listed in Fact~\ref{fact:wpb} are \emph{all} that
we need in this paper.

\shtbs{For proofs we refer to \cite{balt:logi00} and references therein.}

\begin{fact}
\label{fact:wpb}
Let $\F$ be a set functor.
Then the relation lifting $\Fb$ satisfies the following properties, for
all functions $f: S \to S'$, all relations $R,Q \sse S \times S'$, and all 
subsets $T\sse S$, $T' \sse S'$:

(1) $\Fb$ extends $\F$:
$\Fb (\Graph{f}) = \Graph{\F f}$;

(2) $\Fb$ preserves the diagonal:
$\Fb(\Id_{S}) = \Id_{\F S}$;

(3) $\Fb$ commutes with relation converse:
$\Fb (\conv{R}) = \conv{(\Fb{R})}$;

(4) $\Fb$ is monotone: if $R \subseteq Q$ then $\Fb (R) \subseteq \Fb (Q)$;
%\item

(5) $\Fb$ commutes with taking restrictions:
$\Fb (R\bpr_{T\times T'}) = (\Fb R)\bpr_{\F T \times \F T'}$;

(6) $\Fb$ distributes over composition: $\Fb(R \circ Q) = \Fb (R) \circ \Fb (Q)$,
if $\F$ preserves weak pullbacks.
\end{fact}
%%%%%%%%%%%ADDED FACT FOLLOWS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{fact}\label{fact:range}
%	Let $\F: \Set \to \Set$ be a standard. 
%	Then for any function $f:A \to B$ we have 
%	\begin{eqnarray*}
%		\range(\F f) & = & \F \range f
%	\end{eqnarray*}
%\end{fact}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Unfortunately, for the last property of $\Fb$, which is crucial in the proof
of our main result, we need the functor to satisfy a certain categorical
property (the preservation of weak pullbacks).
(The proof that Fact~\ref{fact:wpb} depends on this property goes back
to Trnkov\'a~\cite{trnk:rela77}.)
Fortunately, many set functors in fact do preserve weak pullbacks, which 
guarantees a wide scope for the results in this paper.

\begin{example}
   All functors from example~\ref{ex:BTK} preserve weak pullbacks.
   For the functors $\BT$ and $\K$ this is not difficult to check. 
   A proof for the fact that $\probdist$ is weak pullback preserving
   can be found in~\cite{vinkrut:prob} and~\cite{moss:coal99}. 
   That $\multiset$ is weak pullback preserving is a consequence
   of a more general result in~\ref{gumm:monoid}.

   Furthermore it can be shown that the class of 
   weak pullback preserving functors contains
   all constant functors, and is closed under taking products, coproducts
   and exponentiation. 
\end{example}



\begin{definition}
%\shtbs{polynomial Kripke functors: definition + examples}
\end{definition}



\shtbs{and \ldots}
In particular, one can prove the following fact.

\begin{fact}
All Kripke polynomial functors preserve weak pullbacks.
\end{fact}

Although the precise definition of this categorical property is not relevant
in order to understand this paper, for the interested reader we provide some
details in Remark~\ref{r:wpp} below.

\begin{remark}
\label{r:wpp}
Given two functions $f_{0}: S_{0} \to S$, $f_{1}: S_{1} \to S$, a \emph{weak
pullback} is a set $P$, together with two functions $p_{i}: P \to S_{i}$ such
that $f_{0}\circ p_{0} = f_{1} \circ p_{1}$, and in addition, for every
triple $(Q,q_{0},q_{1})$ also satisfying $f_{0}\circ q_{0} = f_{1}\circ
q_{1}$, there is an arrow $h: Q  \to P$ such that $q_{0} = h\circ p_{0}$ and
$q_{1} = h\circ p_{0}$.
\shtbs{picture to be added}

A functor $\F$ \emph{preserves weak pullbacks} if it transforms every weak
pullback $(P,p_{0},p_{1})$ for $f_{0}$ and $f_{1}$ into a weak pullback for
$\F f_{0}$ and $\F f_{1}$.
(The difference with \emph{pullbacks} is that in the definition of a weak
pullback, the arrow $h$ is not required to be unique.)

A category-theoretically nicer way of formulating Fact~\ref{fact:wpb}(6)
involves the category $\Rel$ the category of sets (as objects) and binary
relations (as arrows). 
A \emdef{relator}, that is, a functor $\mathsf{Q}: \Rel \to \Rel$,
\emdef{extends} a functor $\F: \Set \to \Set$ if $\mathsf{Q} S = \F S$ for 
any object (set) $S$ and $\mathsf{Q} (\Graph{f}) = \Graph{\F f}$ for any
arrow (function) $f$; here $\Graph{f}$ denotes the graph of $f$.
Then one may prove that a set functor $\F$ can be extended to a relator 
iff $\F$ preserves weak pullbacks, and that this extension is unique if its
exists.

Finally, for an example of a functor that does not preserve weak pullbacks,
consider the functor that takes a set $S$ to the set of upward closed subsets
of $(\power S, \subseteq)$, and a function $f$ to its double inverse 
$(f^{-1})^{-1}$.
\end{remark}

From now on all functors appearing in the paper will preserve weak pullbacks.

\subsection{Graph games}
\label{ssec-gg}

Two-player infinite graph games, or \emph{graph games} for short, are defined
as follows.
For a more comprehensive account of these games, the reader is referred 
to {\sc Gr\"adel, Thomas \& Wilke}~\cite{grae:auto02}.

First some preliminaries on sequences.
Given a set $A$, let $A^{*}$, $A^{\om}$ and $A^{\star}$ denote the 
collections of finite, infinite, and all, sequences over $A$, respectively.
(Thus, $A^{\star} = A^{*} \cup A^{\om}$.)
Given $\alpha \in A^{*}$ and $\beta \in A^{\star}$ we define the 
\emph{concatenation} of $\alpha$ and $\beta$ in the obvious way, and we 
denote this element of $A^{\star}$ simply by juxtaposition: $\alpha\beta$.
Given an infinite sequence $\alpha \in A^{\om}$, let $\Inf(\alpha)$ denote
the set of elements $a \in A$ that occur infinitely often in $\alpha$.

%\begin{definition}
A graph game is played on a \emph{board} $B$, that is, a set of \emph{positions}.
Each position $b \in B$ \emph{belongs} to one of the two \emph{players}, $\eloi$
(\'Eloise) and $\abel$ (Ab\'elard).
Formally we write $B = B_{\eloi} \cup B_{\abel}$, and for each position $b$ we 
use $P(b)$ to denote the player $i$ such that $b \in B_{i}$.
Furthermore, the board is endowed with a binary relation $E$, so that each
position $b \in B$ comes with a set $E[b] \sse B$ of \emph{successors}.
Formally, we say that the \emph{arena} of the game consists of a directed
bipartite graph $\bbB = (B_{\eloi} ,  B_{\abel}, E)$.

A \emph{match} or \emph{play} of the game consists of the two players moving
a pebble around the board, starting from some \emph{initial position} $b_{0}$.
When the pebble arrives at a position $b \in B$, it is player $P(b)$'s turn
to move; (s)he can move the pebble to a new position of their liking, but 
the choice is restricted to a successor of $b$.
Should $E[b]$ be empty then we say that player $P(b)$ \emph{got stuck} at
the position.
A \emph{match} or \emph{play} of the game thus constitutes a (finite or 
infinite) sequence of positions $b_{0}b_{1}b_{2}\ldots\ $ such that 
$b_{i}Eb_{i+1}$ (for each $i$ such that $b_{i}$ and $b_{i+1}$ are defined).
A \emph{full play} is either (i) an infinite play or (ii) a finite play in
which the last player got stuck.
A non-full play is called a \emph{partial} play.

The rules of the game associate a \emph{winner} and (thus) a \emph{looser} for
each full play of the game.
A finite full play is lost by the player who got stuck; the winning condition
for infinite games is given by a subset $\Ref$ of $B^{\omega}$ ($\Ref$ is short
for `referee'): our convention is that $\eloi$ is the winner of $\beta \in
B^{\om}$ precisely if $\beta \in \Ref$.
A \emph{graph game} is thus formally defined as a structure $\G = (B_{\eloi}
,  B_{\abel}, E, \Ref)$.
Sometimes we want to restrict our attention to matches of a game with a
certain initial position; in this case we will speak of a game that is 
\emph{initialized} at this position.

Various kinds of winning conditions are known.
In a \emph{parity game}, the set $\Ref$ is defined in terms of a \emph{parity
function} on the board $B$, that is, a map $\Om: B \to \om$ with finite
range.
%; put differently, a parity map on $A$ is a map $\Om: A \to \{ 0,\ldots,
%k \}$ for some natural number $k$.
More specifically, the set $\Ref$ is of the form 
\begin{equation}
\label{e-p-1}
B^{\om}_{\Om} := \{ \beta \in B^{\om} \mid
   \max \{ \Om(b) : b \in \Inf(\beta) \} \mbox{ is even} \}.
\end{equation}

%\shtbs{parity game in table}

A \emph{strategy} for player $i$ is a function mapping partial plays $\beta
= b_{0}\cdots b_{n}$ with $P(b_{n}) = i$ to admissible next positions, that
is, to elements of $E[b_{n}]$.
In such a way, a strategy tells $i$ how to play:
a play $\beta$ is \emph{conform} or \emph{consistent with} strategy $f$ for 
$i$ if for every proper initial sequence $b_{0}\cdots b_{n}$ of $\beta$ with
$P(b_{n}) = i$, we have that $b_{n+1} = f(b_{0}\cdots b_{n})$.
A strategy is \emph{history free} if it only depends on the current 
position of the match, that is, $f(\beta) = f(\beta')$ whenever $\beta$ and
$\beta'$ are partial plays with the same last element (which belongs to the
appropriate player).
Occasionally, it will be convenient to extend the name `strategy' to
arbitrary functions mapping partial plays to positions; in order words, we
allow strategies enforcing \emph{illegal} moves.
In this context, the strategies proper, that is, the ones that dictate
admissible moves only will be called \emph{legitimate}.

A strategy is \emph{winning for player $i$} from position $b \in B$ if it
guarantees $i$ to win any match with initial position $b$, no matter how
the adversary plays --- note that this definition also applies to positions
$b$ for which $P(b) \neq i$.
A position $b \in B$ is called a \emph{winning position} for player $i$, if 
$i$ has a winning strategy from position $b$; the set of winning positions
for $i$ in a game $\G$ is denoted as $\Win_{i}(\G)$.

Parity games form an important game model because they have many attractive
properties, such as \emph{history-free determinacy}.

\begin{fact}
\label{f-2-3}
Let $\G = (B_{\eloi},B_{\abel},E,\Om)$ be a parity graph game. 
Then
%\begin{enumerate}
%\item

1. $\G$ is determined: $B = \Win_{\eloi}(\G) \cup \Win_{\abel}(\G)$.
%\item

2. Each player $i$ has a history free strategy which is winning from 
any position in $\Win_{i}(\G)$.
%\end{enumerate}
\end{fact}

The determinacy of parity games follows from a far more general
game-theoretic result concerning Borel games, due to 
\textsc{Martin}~\cite{mart:bore75}.
The fact that winning strategies in parity games can always be taken to be 
history free, was independently proved in 
\textsc{Mostowski}~\cite{most:game91}
and \textsc{Emerson \& Jutla}~\cite{emer:tree91}.

\subsection{Coalgebra automata and the acceptance game}

Probably the easiest introduction to coalgebra automata involves a
reformulation of the notion of bisimilarity in game-theoretic terms.

It follows from the characterization
(\ref{eq:bis}) that a bisimulation between two coalgebras $\bbA =
\struc{A,\al}$ and $\bbS = \struc{S,\si}$ is nothing but a postfixpoint of
the following operation on the set $\Sb{A \times S}$ of binary relations
between $A$ and $S$:
\[
Z \mapsto \{ (a,s) \in A \times S \mid 
(\al(a),\si(s)) \in \Fb(Z) \}.
\]
By monotonicity of relation lifting, this operation is monotone, and thus
it is an immediate consequence of standard fixpoint theory that there is a
largest bisimulation between the two coalgebras, which is given as the union
of all bisimulations between $\bbA$ and $\bbS$.
Furthermore, this largest bisimulation has a nice \emph{game-theoretic}
characterization.

For an informal description of this game, 
%let $\bbS = (S,\si)$ and $\bbS' =
%(S',\si')$ be two $\F$-coalgebras for some set functor $\F$.
%The \emph{bisimulation game} $\B(\bbS,\bbS')$ between $\bbS$ and $\bbS'$ is
%defined as a graph game between two players $\eloi$ and $\abel$.
%The positions for these players are respectively the sets $B_{\eloi} :=
%S \times S'$ and $B_{\abel} := \power(S \times S')$.
%The
the admissible moves of the players are given as follows:
\begin{itemize}
\item
in position $(a,s)$, $\eloi$ may choose a \emph{local bisimulation} for 
$a$ and $s$, i.e., a relation $Z \sse A \times S$ satisfying
$(\al(a),\si(s)) \in \Fb Z$;
\item
in position $Z \sse A \times S$, $\abel$ may choose any element $(t,t')$ 
of $Z$.
\end{itemize}
Finally, the winning conditions for infinite matches of this game are very
simple: if $\eloi$ manages to survive all finite stages of a match, she is
declared the winner of the resulting infinite match.

This bisimilarity game can be formulated as a graph game with a very simple
parity winning condition.

\begin{definition}\label{def:bisgame}
Let $\F$ be a set functor, and let $\bbS = (A,\al)$ and $\bbS = (S,\si)$
be two $\F$-coalgebras.
The \emph{bisimilarity game} $\B(\bbA,\bbS)$ associated with $\bbA$ and
$\bbS$ is the parity graph game $(B_{\eloi},B_{\abel},E,\Om)$ with
\[\begin{array}{lll}
   B_{\eloi} &:=& A \times S
\\ B_{\abel} &:=& \Sb{A \times S},
\end{array}\]
while $E$ and $\Om$ are given in Table~\ref{tb:1}.
Positions of the form $(a,s) \in A \times S$ are called \emph{basic}.
\begin{table*}[t]
\begin{center}{\small 
\begin{tabular}[b]{|l|c|l|c|}
\hline
Position: $b$ & $P(b)$ & Admissible moves: $E[b]$ & $\Om(b)$ \\ \hline
$(a,s) \in  A \times S$           & $\eloi$ &
   $\{ Z \in \Sb{A \times S} \mid (\al(a),\si(s)) \in \Fb Z \}$    & 0 \\
$Z \in \Sb{A \times S}$           & $\abel$ & $Z$             & 0 \\ \hline
\end{tabular}
}\end{center}
\caption{Acceptance game for an $\F$-automaton}
\label{tb:1}
\end{table*}
The set of winning positions for $\eloi$ in this game is denoted as
$\Win_{\eloi}(\B(\bbA,\bbS))$, or $\Win_{\eloi}$ if no confusion is likely.
\end{definition} 

\begin{remark}
We leave it to the reader to verify that
\[
(a,s) \in \Win_{\eloi}(\B) \mbox{ iff } \bbA,a \bis \bbS,s.
\]
The key observation here is that the relation 
$\{ (a,s) \in A \times S \mid (a,s) \in \Win_{\eloi}(\B)\}$ is the largest
bisimulation between $\bbA$ and $\bbS$.
\end{remark}

In order to make the key observation in understanding coalgebra automata,
we take a slightly \emph{different perspective} on the bisimilarity game.
The point is to think of one structure ($\bbA$) as %an automaton 
\emph{classifying} the other one ($\bbS$).
This conceptual removal of the symmetry between the two structures,
enables us think of $\bbA$ as an \emph{automaton} operating on $\bbS$,
and of the game as an \emph{acceptance game} rather than as a comparison
game.
But from this perspective it is natural to impose some modifications on 
$\bbA$, making it resemble the standard concept of an automaton more
closely:

To start with, the state space $A$ of $\bbA$ is required to be finite,
and $\bbA$ will have a fixed \emph{initial state} $\ai \in A$.

Second, some infinite matches may be won by $\abel$.
This can easily be implemented as follows.
With each infinite match of the game we may associate an infinite stream of
\emph{basic positions} of the form $(a,s) \in A \times S$, and thus an
infinite stream of states from $A$. 
Hence, the winning conditions in the game can be formulated using a subset
$\Acc \sse A^{\om}$.
And since $A$ is finite we may use more specific conditions; for instance, 
a parity condition can be formulated by a map $\Om: A \to \om$.

And finally, we may ntroduce \emdef{nondeterminism} or even \emph{alternation}
on $\bbA$.
Here the idea is that, whereas in a coalgebra $\bbA = \struc{A,\al}$,
the `successor object' of a state $a \in A$ is fixed as $\al(a) \in \F A$,
we may now allow $\eloi$ to dynamically \emph{choose} this object from some 
\emph{set} $\De(a) \in \power(\F A)$ of objects in $\F A$.
Or, the `successor object' of $a \in A$ may be dynamically determined via
some game-theoretic interaction between the \emph{two} players.

Putting these observations together, we arrive at the following definition
of \textsc{Venema}~\cite{vene:auto04}.

\begin{convention}{\rm
In the sequel we will frequently denote the power set $\power S$ of a 
set $S$ by either $\pwE S$ or $\pwA S$.
This notation indicates that we are in a game-theoretic context, where $X
\in \power_{i} S$ means that $X$ represents a collection of possible moves,
and that $i$ is the player who may choose an element from $X$.
}\end{convention}

\begin{definition}\label{def:Fautomaton}
Let $\F$ be some set functor.
An (alternating) {\em $\F$-automaton} is a quadruple $\bbA = (A,\ai,\Delta,
\Acc)$ with $A$ some finite set of objects called {\em states}, $\ai \in A$ the 
{\em initial state}, $\Delta: A \to \power \power \F A$ the {\em transition 
function} and $\Acc \sse A^{\om}$ the \emph{acceptance condition}.
An $\F$-automaton is called {\em nondeterministic} if each member of each 
$\Delta(a)$ is a singleton set.

A \emph{parity} $\F$-automaton is an $\F$-automaton $\bbA = (A,\ai,\Delta,
\Acc)$ where $\bbA$ is given by some parity condition $\Om: A \to \omega$;
such a structure will usually be denoted as $\bbA = (A,\ai,\Delta,\Om)$.
\end{definition}

$\F$-automata are designed to accept or reject pointed $\F$-coalgebras.
The acceptance condition is formulated in terms of a graph game.
For an informal description of this game, the first observation is that 
matches of this game proceed in \emph{rounds} that start and end in a 
\emph{basic position} of the form $(s,a) \in S \times A$.
From such a basic position $(s,a)$, play proceeds as follows:
\begin{itemize}
\item 
$\eloi$ picks an element $\Phi \in \De(a)$, making $(s,\Phi) \in S
\times \pwA \F A$ the next position.
\item
$\abel$ picks $\phi \in \Phi$, moving to position $(s,\phi) \in S
\times \F A$.
\end{itemize}
Note that this interaction between $\eloi$ and $\abel$ has fixed the 
`successor' $\phi \in \F A$ of $a$, whereas the `successor' $\si(s)$
of $s$ was determined from the outset.
\begin{itemize}
\item
$\eloi$ picks a `local bisimulation' $Y$ for $\phi$ and $\si(s)$, that is, 
a binary relation $Y \sse S \times A$ such that $(\si(s),\phi) \in \Fb Y$.
This relation $Y_{s,\phi}$ is itself the new position.
\item
$\abel$ chooses a pair $(t,b) \in Y$ as the next basic position.
\end{itemize}
In the sequel we will refer to the first two moves in the round of the game
as the \emph{static} part of the round (static because the match does not
pass to another state in the coalgebra), and to the last two moves as the 
\emph{dynamic} or \emph{coalgebraic} stage of the round.

For the winning conditions, recall that finite matches are lost by the
player who get stuck. 
For infinite matches, consider an arbitrary such match:
\[
\mu \;=\; 
(s_{0},a_{0})(s_{0},\Phi_{0})(s_{0},\phi_{0})Y_{0}
(s_{1},a_{1})(s_{1},\Phi_{1})(s_{1},\phi_{1})Y_{1}
(s_{2},a_{2})\ldots
\]
Clearly, $\mu$ induces an infinite sequence of basic positions
\[
(s_{0},a_{0})(s_{1},a_{1})(s_{2},a_{2})\ldots
\]
and, thus, an infinite sequence of states in $A$:
\[
\mu\bpr_{A}:= a_{0}a_{1}a_{2}\ldots
\]
Now the winner of the match is determined by whether $\mu\bpr_{A}$ belongs
to the set $\Acc$ or not.

\begin{definition}\label{def:accgame}
Let $\bbA = (A,\ai,\De,\Acc)$ be an $\F$-automaton, and let $\bbS = (S,\si)$ be
an $\F$-coalgebra.
The \emph{acceptance game} $\G(\bbA,\bbS)$ associated with $\bbA$ and $\bbS$
is the graph game $(B_{\eloi},B_{\abel},E,\ovl{\Acc})$ with
\[\begin{array}{lllll}
   B_{\eloi} &:=& S \times A           &\cup& S \times \F A
\\ B_{\abel} &:=& S \times \power \F A &\cup& \Sb{S \times A},
\end{array}\]
where $E$ is given in Table~\ref{tb:2}.
Positions of the form $(a,s) \in A \times S$ are called \emph{basic}.
\begin{table*}[t]
%\label{tb:2}
\begin{center}{\small 
\begin{tabular}[b]{|l|c|l|}
\hline
Position: $b$ & $P(b)$ & Admissible moves: $E[b]$  \\ \hline
$(s,a) \in  S \times A$           & $\eloi$ &
   $\{ (s,\Phi) \in S \times \Sb{\F A} \mid \Phi \in \De(a) \}$  \\
$(s,\Phi) \in S \times \Sb{\F A} $  & $\abel$ &
   $\{ (s,\phi) \in S \times \F A \mid
       \phi \in \Phi \}$               \\
$(s,\phi) \in S \times \F A$ & $\eloi$ &
   $\{ Z \in \Sb{S \times A} \mid (\si(s),\phi) \in \Fb Z \}$    \\
$Z \in \Sb{S \times A}$           & $\abel$ & $Z$              \\ \hline
\end{tabular}
}\end{center}
\caption{Acceptance game for an $\F$-automaton}
\label{tb:2}
\end{table*}

For the winning conditions of $\G(\bbA,\bbS)$, observe that every infinite
match $\mu$ induces an infinite sequence $\mu\bpr_{A} := a_{0}a_{1}a_{2}\ldots
\in A^{\om}$.
Now the winner of $\mu$ is $\eloi$ if $\mu_\bpr{A} \in \Acc$, and $\abel$ 
otherwise.

The set of winning positions for $\eloi$ in this game is denoted as
$\Win_{\eloi}(\G(\bbA,\bbS))$, or $\Win_{\eloi}$ if no confusion is likely.
$\bbA$ \emph{accepts} the pointed $\F$-coalgebra $(\bbS,s)$ if $(s,\ai) \in 
\Win_{\eloi}$.
\end{definition} 

%% 
 % \begin{definition}\label{def:accgame}
 % Let $\bbA = (A,\ai,\De,\Om)$ be an $\F$-automaton, and let $\bbS = (S,\si)$ be
 % an $\F$-coalgebra.
 % The \emph{acceptance game} $\G(\bbA,\bbS)$ associated with $\bbA$ and $\bbS$
 % is the parity graph game $(B_{\eloi},B_{\abel},E,\ovl{\Om})$ with
 % \[\begin{array}{lllll}
 %    B_{\eloi} &:=& S \times A           &\cup& S \times \F A
 % \\ B_{\abel} &:=& S \times \power \F A &\cup& \Sb{S \times A},
 % \end{array}\]
 % while $E$ and $\ovl{\Om}$ are given in Table~\ref{tb:2}.
 % \begin{table*}[t]
 % %\label{tb:2}
 % \begin{center}{\small 
 % \begin{tabular}[b]{|l|c|l|c|}
 % \hline
 % Position: $b$ & $P(b)$ & Admissible moves: $E[b]$ & $\ovl{\Om}(b)$ \\ \hline
 % $(s,a) \in  S \times A$           & $\eloi$ &
 %    $\{ (s,\Phi) \in S \times \Sb{\F A} \mid \Phi \in \De(a) \}$ & $\Om(a)$ \\
 % $(s,\Phi) \in S \times \Sb{\F A} $  & $\abel$ &
 %    $\{ (s,\phi) \in S \times \F A \mid
 %        \phi \in \Phi \}$              & 0 \\
 % $(s,\phi) \in S \times \F A$ & $\eloi$ &
 %    $\{ Z \in \Sb{S \times A} \mid (\si(s),\phi) \in \Fb Z \}$    & 0 \\
 % $Z \in \Sb{S \times A}$           & $\abel$ & $Z$             & 0 \\ \hline
 % \end{tabular}
 % }\end{center}
 % \caption{Acceptance game for an $\F$-automaton}
 % \label{tb:2}
 % \end{table*}
 % The set of winning positions for $\eloi$ in this game is denoted as
 % $\Win_{\eloi}(\G(\bbA,\bbS))$, or $\Win_{\eloi}$ if no confusion is likely.
 % $\bbA$ \emph{accepts} the pointed $\F$-coalgebra $(\bbS,s)$ if $(s,\ai) \in 
 % \Win_{\eloi}$.
 % \end{definition} 
 %%

\begin{remark}
\btbs
\item
notation for nondeterministic automata
\item
that this is nothing new
\etbs
\end{remark}

\begin{remark}
It is clear from the definition of $\ovl{\Om}$ that only the \emdef{basic} 
positions of a match, i.e., positions of the form $(s,a) \in S \times A$, are 
relevant to determine the winner of the match.
Accordingly, in the sequel we will frequently represent a match of the game 
by the sequence of basic positions visited during the match.
\end{remark}

It is easy to see that the acceptance games associated with \emph{parity} 
automata, are parity games. 
(Simply define the priority of a basic position $(s,a)$ as $\ovl{\Om}(s,a)
:= \Om(a)$, putting $\ovl{\Om}(p) := 0$ for all other positions.)
But parity games are known to enjoy a strong form of determinacy: in any
position of the game board either $\eloi$ or $\abel$ has a history-free
winning strategy.
Therefore we can focus on $\eloi$'s history-free strategies.

\begin{definition}\label{def:eloistrategy}
Given an $\F$-coalgebra $(S,\sigma)$ and a parity $\F$-automaton $\bbA$ a 
{\em positional strategy} of $\eloi$ is a pair of functions 
\[
(\Phi:S \times A \to \pwA \F A, \; Z:S \times \F A \to \Sb{S \times A}).
\]
Such a strategy is \emdef{legitimate} at a position if it maps the position 
to an admissible next position.
A partial strategy of the kind $\Phi: S \times A \to \power \F A$ will often
be represented as a map $\Phi: S \to (\power \F)^{A}$; values of this map 
will be denoted as $\Phi_s$, etc.
\end{definition}

\newpage

In the paper we will also need a slight variation of an $\F$-automaton.
For any set $C$, a $C$-coloring of a coalgebra $\bbS$ is a map $\ga: S \to 
C$; the $C$-colored $\F$-coalgebra  $\bbS \oplus \ga := \struc{S,\ga,\si}$
can be identified with the $C \times \F$-coalgebra $\struc{S,\langle \ga,\si 
\rangle}$.

\shtbs{reconsider chromatic automata}

\begin{definition}\label{def:chromatic}
Let $C$ be a finite set.
A \emph{$C$-chromatic $\F$-automaton} is a quintuple $\bbA = (A,\ai,C,\De,\Om)$ 
such that $\De: A \times C \to \power\power \F A$ (and $A$, $\ai$, and $\Om$ 
are as before).
Given such an automaton and a $C \times \F$-coalgebra $\bbS = (S,\ga,\si)$, 
the acceptance game $\G_{C}(\bbA,\bbS)$ is defined as the acceptance game
for $\F$-automata with the only difference that $\eloi$ has to
move from a position $(s,a)$ to a position $(s,\Phi)$ such
that $\Phi \in \Delta(a,\gamma(s))$.
\phantom{bla}
%in a very similar way as before,
%witnessed by table~\ref{tb:3}.
%\begin{table*}
%\begin{center}{\small 
%\begin{tabular}[b]{|l|c|l|c|}
%\hline
%Position: $b$ & $P(b)$ & Admissible moves: $E[b]$    & $\ovl{\Om}(b)$  \\ \hline
%$(s,a) \in  S \times A$           & $\eloi$ &
%   $\{ (s,\Phi) \in S \times \Sb{\F A} \mid \Phi \in \De(a,\ga(s)) \}$ &
%   $\Om(a)$ \\
%$(s,\Phi) \in S \times \Sb{\F A} $  & $\abel$ &
%   $\{ (s,\phi) \in S \times \F A \mid
%       \phi \in \Phi \}$      & 0 \\
%$(s,\phi) \in S \times \F A$ & $\eloi$ &
%   $\{ Z \in \Sb{S \times A} \mid (\si(s),\phi) \in \Fb Z \}$   & 0 \\
%$Z \in \Sb{S \times A}$           & $\abel$ & $Z$            & 0 \\ \hline
%\end{tabular}
%}\end{center}
%\caption{Acceptance game for a chromatic $\F$-automaton}
%\label{tb:3}
%\end{table*}
%\shtbs{finite words}
\end{definition}

\begin{example}
The well-known word, tree and graph automata are instantiations of this
notion.
Infinite words over an alphabet $C$ can be seen as $C$-colored coalgebras
over the identity functor $\Id$, so parity automata for infinite $C$-words
correspond to $C$-chromatic $\Id$-automata. 
Likewise, $C$-chromatic $\Id \times \Id$-automata correspond to automata on
infinite binary trees, and $C$-chromatic $\power$-automata correspond to 
amorphous tree or graph automata, with $C$ in all cases denoting the 
\emph{alphabet}.

For each functor $\F$ mentioned above, our notion may also take care of
the automata operating on the corresponding \emph{finite} objects.
For instance, finite words over $C$ may be taken as $C$-colored coalgebras
for the functor $\{ \downarrow \} + \Id$, with $\downarrow$ denoting 
termination.
\end{example}
%It was shown in  that $C$-chromatic $\F$-automata and 
%$C \times \F$-automata have the same recognizing power.
We need the following fact from \cite{vene:auto04}.
\begin{fact}
\label{f:2:1}
With any $C \times \F$-automaton $\bbA$ we may associate a $C$-chromatic 
$\F$-automaton $\bbA_C$, the {\em $C$-chromatic $\F$-companion} of $\bbA$, such 
that $\bbA$ and $\bbA_C$ accept the same $C \times \F$-coalgebras. 
\end{fact}

\subsection{Mathematical preliminaries}

\btbs
\item
range of relation
\etbs

